IntelliCircos: A Data-driven and AI-powered Authoring Tool for Circos Plots

Genomics data is essential in biological and medical domains, and bioinformatics analysts often manually create circos plots to analyze the data and extract valuable insights. However, creating circos plots is complex, as it requires careful design for multiple track attributes and positional relationships between them. Typically, analysts often seek inspiration from existing circos plots, and they have to iteratively adjust and refine the plot to achieve a satisfactory final design, making the process both tedious and time-intensive. To address these challenges, we propose IntelliCircos, an AI-powered interactive authoring tool that streamlines the process from initial visual design to the final implementation of circos plots. Specifically, we build a new dataset containing 4396 circos plots with corresponding annotations and configurations, which are extracted and labeled from published papers. With the dataset, we further identify track combination patterns, and utilize Large Language Model (LLM) to provide domain-specific design recommendations and configuration references to navigate the design of circos plots. We conduct a user study with 8 bioinformatics analysts to evaluate IntelliCircos, and the results demonstrate its usability and effectiveness in authoring circos plots.

==> egbibsample-backup.tex <==
@String{cgforum = "Computer Graphics Forum"}
@String{tog = "ACM TOG"}

@article{Buhmann:1998:DCQ,
	AUTHOR = {J. M. Buhmann and D. W. Fellner and M. Held and J.
		Ketterer and J. Puzicha},
	TITLE = {Dithered Color Quantization},
	JOURNAL = cgforum,
	EDITOR = {N. Ferreira and M. G\"{o}bel},
	VOLUME = {17},	NUMBER = {3},
	MONTH = Sep,	YEAR = {1998},	PAGES = {C219-C231},
	DOI = {10.1111/1467-8659.00269},
  NOTE = {(Proc. Eurographics'98)
	       \httpsAddr{//diglib.eg.org/handle/10.2312/8491}} }

@ARTICLE{Fellner-Helmberg93,
	AUTHOR = {Fellner, Dieter W. and Helmberg, Christoph},
	TITLE = {Robust Rendering of General Ellipses and Elliptical Arcs},
	JOURNAL = tog,
	VOLUME = {12},	NUMBER = {3},
	MONTH = Jul,	YEAR = {1993},	PAGES = {251-276},
  DOI= {10.1145/169711.169704}
  }

@BOOK (FolDamFeiHug.etal93,
	AUTHOR = {Foley, James D. and van Dam, Andries and
		Feiner, Stephen K. and Hughes, John F. and Phillips, R.},
	TITLE = {Introduction to Computer Graphics},
	PUBLISHER = {Addison-Wesley},
	YEAR = {1993} )

@ARTICLE{Kobbelt97-USHDR,
	author = {L. Kobbelt and M. Stamminger and H.-P. Seidel},
	title = {Using Subdivision on Hierarchical Data to Reconstruct Radiosity
		Distribution},
	JOURNAL = cgforum,
	volume = 16,	number = 3,	pages = {C347-C355},
	year = 1997,
	DOI = {10.1111/1467-8659.16.3conferenceissue.36},
	note = {(Proc. Eurographics'97)
	       \httpsAddr{//diglib.eg.org/handle/10.2312/8393}} }

@INPROCEEDINGS{Lafortune97-NARF,
	author = {Eric P. Lafortune and Sing-Choong Foo and Kenneth E. Torrance and
		Donald P. Greenberg},
	title = {Non-Linear Approximation of Reflectance Functions},
	booktitle = {Proc. SIGGRAPH '97},
	volume = 31,	pages = {117-126},
	year = 1997,
	DOI = {10.1145/258734.258801}
  }

@ARTICLE (Lous90,
	AUTHOR = {Y. Le Lous},
	TITLE = {Report on the {F}irst {E}urographics {W}orkshop on {V}isualization in
		{S}cientific {C}omputing},
	JOURNAL = cgforum,
	VOLUME = {9},	NUMBER = {4},
	MONTH = dec,	YEAR = {1990},	PAGES = {371-372},
  DOI= {10.1111/j.1467-8659.1990.tb00430.x}
  )

@ARTICLE (Seidel93,
	AUTHOR = {Seidel, Hans-Peter},
	TITLE = {Polar Forms for Geometrically Continuous Spline Curves of
		Arbitrary Degree},
	JOURNAL = tog,
	VOLUME = {12},	NUMBER = {1},
	MONTH = Jan,	YEAR = {1993},	PAGES = {1-34},
  DOI= {10.1145/169728.169726}
  )


